Utility-Driven Speculative Decoding for Mixture-of-Experts

GPU memory bandwidth is the main bottleneck for low-latency Large Language Model (LLM) inference. Speculative decoding leverages idle GPU compute by using a lightweight drafter to propose K tokens, which the LLM verifies in parallel, boosting token throughput. In conventional dense LLMs, all model weights are fetched each iteration, so speculation adds no latency overhead. Emerging Mixture of Experts (MoE) models activate only a subset of weights per token, greatly reducing data movement. However, we show that speculation is ineffective for MoEs: draft tokens collectively activate more weights, increasing data movement and verification time by 2-3x. When token throughput gains fail to offset this overhead, speculation causes slowdowns up to 1.5x, making it infeasible. Even when useful, the optimal K varies by task, model, and even between requests and iterations. Thus, despite widespread use in dense LLMs, speculation remains impractical in leading MoEs. We present Cascade, a utility-driven framework that selectively enables speculation to avoid slowdowns and dynamically tunes K to accelerate MoE serving. Cascade uses a lightweight metric, speculation utility, the ratio of token gains to verification cost, which shows iteration-level locality, enabling periodic decisions via short test and longer set phases. For each request, Cascade disables speculation if utility drops below one during testing, and when utility exceeds one, tests multiple K-values to choose the utility-maximizing K for the set phase. We implement Cascade in vLLM and evaluate it on five popular MoEs with workloads spanning code, math, extraction, and mixed tasks. Cascade limits slowdown to 5% (vs. 1.5x) and improves throughput by 7-14% over static K, making speculative decoding practical for MoEs.

==> sections/NAN.dynamic_spec_decode.tex <==
\section{\TheName: Cost-Aware Speculative Decoding}

==> sections/NAN.restricting_experts.tex <==
\section{Verify Efficiently: Adaptive Expert Sets}

==> todo.tex <==
P1: all of the content and experiments need to be in in [DONE]
P2: focus on first 6 pages [4 PM]
P3: harp on data-movement problem 
P4: harp on utility in abstract, intro, motivation
P5: check 15\% and 5\% max slowdown claim in Intro
P6: update hyperparam sens result
P7: update spec-utility plots and remove eagle

For Sec 2.2:
- for spec tokens in spec-decode, show usage of same experts and we lose some, win some
- fig 1c is dense, make it simpler (only 3-4 examples)
- fig 18: y-axis is TPOT speedup. Include K=1, K=2 bars. make it full text width. increase height and start from y=0.
- sec2: ETR shows temporal locality across iterations. using few tokens for the remaining tokens is a good idea.
- fig 4: hatch verify bars. green vs red is not visible. 


Fig-4: y axis starts at arbitrary value.  Lets start at 0. Given the wide range, there is no good reason to start at 0.3.

Fig-3:  Is there a checkmark and cross missing after the Accepted?

Fix captions on Page-10
